Analysis of GSI HADES beamline configuration space

The High-Energy Beam Transport system of GSI Campus is a complex system of interconnected beamlines between SIS18 synchrotron and multiple experimental stations and storage rings. This system is designed to be flexible and each experimental station can be reached by several beam paths. The quadrupole settings must fulfill constraints due to the beamline acceptance, limitations of the installed magnets and experimental requirements. The number of degrees of freedom is large and leaves operators with a vast number of possible optics configurations. The choice of a particular configuration is often a matter of compromises, very specific requirements, operational experience and personal style. Once a satisfying configuration is found, the space of possible solutions is usually not explored any further. Here the Monte Carlo method is used to probe the space of all possible beamline optics configurations. The focus is on a particular section, the HADES beamline, because this is one of the most demanding lines due to high beam intensities required by the experiment. The presented analysis gives an overview of the possible settings, insight into beamline potential and flexibility and supports the choice of an optimal operational setting.

==> sub/matching_convergence.tex <==
\section{Convergence of matching process}
% jupyter 0.4
Here we look at the distance between the initial, randomly chosen set of k-values and the final one, after the matching procedure.
It must be stressed that only a small fraction of the randomly-chosen set of k-values converge. This is a property
of the beam line but also of the minimization algorithm.
In our exercise this fraction was only 0.034\%. 
In other cases the matching process ends, after a predefined maximum number of steps (?), without convergence.

Here we show result for a simply 21-dimensional euclidean distance between initial k-value point and the final one.
The left plot in Figure \ref{fig:euclidean_distance} shows the distance distribution. 
The right plot shows the PC phase space colored according to the movement of the configurations during the matching process.
Read areas are areas which loose configurations during the matching and blue areas are 'attractors'.
The plot is basically a difference of the maps in Figure \ref{fig:pca_mountains}


\begin{figure}[htb]
   \centering
   \includegraphics[width=.45\textwidth]{plots/if_euclidean.png}   
   \includegraphics[width=.45\textwidth]{plots/pca_attractors_10k_nist.png} % 09
   \caption{Distribution of euclidean distances between the initial and final kL-values.
Right plot: read areas are areas where the initial models are leaving, blue areas are attractors.   
   }
   \label{fig:euclidean_distance}
\end{figure}


==> sub/microstructure_old.tex <==
In order to investigate the configuration space microstucture additiona configurations were generated in 21-dimensional hypespherical shells around each good configuration. The difference between inner and outer radius of each shell is $\rm 0.001~m^{-2}$.
 No matching procedure was performed, so results are purely MC sampling.

The number and spread of good configurations (lets call them subconfigurations) found this way gives a good estimation of the shape of the local configuration space. The plots in Figure \ref{fig:disp_size} show a distribution of number of subconfigurations and a maximum distance of a subconfiguration from the main configuration. Significant fraction of configurations have no or a very few subconfigurations around them. The maximum distance between a valid configuration and subconfigurations reach about $\rm 0.025~m^{2}$. This distance is still at least a factor 10 smaller than a distance between various configurations (see Figure \ref{fig:k1_distances}). Configurations with large number of subconfigurations form kind of local clumps of favorable configuration space.


 The volume occupied by configurations can be calculated from Equation:
 (Mean-Value MonteCarlo)
 
 \begin{equation}
     V_{clump}=\Sigma_{i=0}^{N_{shell}} (\frac{N_{i,good}}{N_{i,total}}*V_{i})
 \end{equation}

Where the $V_{i}$ is volume of a given shell, $N_{i,good}$ is the number of configurations fulfilling the matching conditions and 
$N_{i,total}$ is number of attempted configurations.

These results do not detect all good configurations, however, quite likely a major part of {\it clumps} are detected. It is not excluded that there are thin filaments made of good configurations which connect the {\it clumps}.

